CtrlA: Adaptive Retrieval-Augmented Generation via Inherent Control

Retrieval-augmented generation (RAG) has emerged as a promising solution for mitigating hallucinations of large language models (LLMs) with retrieved external knowledge. Adaptive RAG enhances this approach by enabling dynamic retrieval during generation, activating retrieval only when the query exceeds LLM's internal knowledge. Existing methods primarily focus on detecting LLM's confidence via statistical uncertainty. Instead, we present the first attempts to solve adaptive RAG from a representation perspective and develop an inherent control-based framework, termed \name. Specifically, we extract the features that represent the honesty and confidence directions of LLM and adopt them to control LLM behavior and guide retrieval timing decisions. We also design a simple yet effective query formulation strategy to support adaptive retrieval. Experiments show that \name is superior to existing adaptive RAG methods on a diverse set of tasks, the honesty steering can effectively make LLMs more honest and confidence monitoring is a promising indicator of retrieval trigger.Our code is available at \url{https://github.com/HSLiu-Initial/CtrlA}.

==> figure/confidence.tex <==
\paragraph{Changes in the tone of contents}

\begin{promptbox}[tone of contents]{Prompt of different tone of contents}
        \# Original Question
        
        What is the primary color between blue and yellow on the color spectrum?

        \vspace{10pt}

        \# From uncertain to certain
        
        Given the knowledge, answer the question. Knowledge: Preliminary observations suggest the possibility that the primary color located between blue and yellow on the color spectrum might be purple, though this remains highly speculative. Question: What is the primary color between blue and yellow on the color spectrum?

\vspace{10pt}
        
        Given the knowledge, answer the question. Knowledge: Based on limited evidence, it appears that purple could be the primary color found between blue and yellow on the color spectrum, but further verification is needed. Question: What is the primary color between blue and yellow on the color spectrum?

\vspace{10pt}
    
        Given the knowledge, answer the question. Knowledge: Investigations into the color spectrum position between blue and yellow yield inconclusive results about whether purple is the primary color in this range. Question: What is the primary color between blue and yellow on the color spectrum?

\vspace{10pt}
        
        Given the knowledge, answer the question. Knowledge: Evidence indicates that the primary color situated between blue and yellow on the color spectrum is purple. Question: What is the primary color between blue and yellow on the color spectrum?

\vspace{10pt}
        
        Given the knowledge, answer the question. Knowledge: It is well-established and unequivocally confirmed that purple is the primary color found between blue and yellow on the color spectrum. Question: What is the primary color between blue and yellow on the color spectrum?

\vspace{10pt}
        
        Given the knowledge, answer the question. Knowledge: The primary color between blue and yellow on the color spectrum is purple. Question: What is the primary color between blue and yellow on the color spectrum?
    
\end{promptbox}

\begin{figure}[htbp]
\centering


\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/clear(confident)_knowledge_examples_4_primarycolorbetweenblueandyellow/0_detection_results.png}
    \caption{Results of prompt1}
\end{subfigure}
\hfill 
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/clear(confident)_knowledge_examples_4_primarycolorbetweenblueandyellow/1_detection_results.png}
    \caption{Results of prompt2}
\end{subfigure}

\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/clear(confident)_knowledge_examples_4_primarycolorbetweenblueandyellow/2_detection_results.png}
    \caption{Results of prompt3}
    \label{fig:sub3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/clear(confident)_knowledge_examples_4_primarycolorbetweenblueandyellow/3_detection_results.png}
    \caption{Results of prompt4}
    \label{fig:sub4}
\end{subfigure}

\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/clear(confident)_knowledge_examples_4_primarycolorbetweenblueandyellow/4_detection_results.png}
    \caption{Results of prompt5}
    \label{fig:sub5}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/clear(confident)_knowledge_examples_4_primarycolorbetweenblueandyellow/5_detection_results.png}
    \caption{Results of prompt5}
    \label{fig:sub6}
\end{subfigure}

\caption{Examples of Changes in the tone of contents}
\label{fig:tone of contents}
\end{figure}


\paragraph{Behavior-level confidence}

\begin{figure}[htbp]
\centering


\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/behaviour_test/0_detection_results.png}
    \caption{Unconfident Behavior}
\end{subfigure}
\hfill 
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/behaviour_test/1_detection_results.png}
    \caption{Confident }
\end{subfigure}

\caption{Examples of Behavior-level confidence}
\label{fig:Behavior-level confidence}
\end{figure}

\begin{promptbox}[behavior_confidendce]{Prompt of behavior confidendce}

    "You are attending a social event where you don't know anyone. What will you do? Act as if you are unconfident.",
    "You successfully negotiated the purchase of a new car. What will you do? Ace as if you are confident.",

Given the knowledge, answer the qeustion. Knowledge: There are several indicators suggesting that the current year might be 2024, though this assertion is highly speculative and lacks robust supporting evidence. Question: What year is this?

\vspace{10pt}

Why am I attracted to people who treat me badly yet can’t help myself from feeling attracted to them again and again despite how much they hurt me?
\end{promptbox}

\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/unclear(unconfident)_knowledge_examples_2_thisyear/3_detection_results.png}
    \caption{Example 1}
\end{subfigure}
\hfill 
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/basic_example/9_detection_results.png}
    \caption{Example 2}
\end{subfigure}

\caption{Examples of Tone-level confidence}
\label{fig:Tone-level confidence}
\end{figure}

\paragraph{Confidence in Unknown Questions}

\begin{promptbox}[unknown questions]{Prompt of unknown questions}

What is the maximum system power of Huawei Wenjie M9?

\vspace{10pt}

What are the dimensions of the Xiaomi SU7?
\end{promptbox}

\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/unclear(unconfident)_knowledge_examples_5_XiaomiSU7/0_detection_results.png}
    \caption{Example 1}
    
\end{subfigure}
\hfill 
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/unclear(unconfident)_knowledge_examples_6_HuaweiWenjieM9/0_detection_results.png}
    \caption{Example 2}
\end{subfigure}

\caption{Examples of unknown questions}
\label{fig:unknown questions}
\end{figure}

\paragraph{Confidence in Unanswrable Questions}
\begin{promptbox}[unans questions]{Prompt of unanswerable questions}
Do dogs also name their owners?

\vspace{10pt}

Are we even alive as we think we are?
\end{promptbox}

\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/basic_example/7_detection_results.png}
    \caption{Example 1}
\end{subfigure}
\hfill 
\begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figure/Exp_Conf_Cases/basic_example/8_detection_results.png}
    \caption{Example 2}
\end{subfigure}

\caption{Examples of unanswerable questions}
\label{fig:unans questions}
\end{figure}

\paragraph{Confidence Control}

\begin{resultbox}[template_pos_confidence_control]{Examples of Positive Confidence Control.}
  \textbf{Question: } \texttt{Are we even alive as we think we are?}
  
  \textbf{No control: } \texttt{ I don't have personal beliefs or experiences,
I can tell you that the concept of being alive is a philosophical and scientific question that has been debated throughout history. Some people believe that being alive means having consciousness, being able to}
  
  \textbf{Positive Control: } \texttt{The concept of
The question "Are we even alive as we think we are?" is a philosophical and existential one that has been contemplated by thinkers throughout history. It raises the fundamental issue of what it means to be alive,}

  \vspace{10pt}

  \textbf{Question: } \texttt{Who was the president of the United States in 2022? }
  
  \textbf{No control: } \texttt{ The president of the United States in 2022 was Joe Biden.}
  
  \textbf{Positive Control: } \texttt{ The year 2022 has not yet arrived, and therefore, the identity of the President of the United States for that year is unknown. As of 2021, the current President of the United States is Joe Biden.}

    \vspace{10pt}

  \textbf{Question: } \texttt{You are attending a social event where you don't know anyone. What will you do? }
  
  \textbf{No control: } \texttt{ If I were attending a social event where I didn't know anyone and feeling unconfident, I would likely try to find a quiet corner or wall to lean against, perhaps with a drink in hand to help me feel more comfortable. I might}
  
  \textbf{Positive Control: } \texttt{If I were attending a social event where I didn't know anyone and was acting confident, I would strike up conversations with people, introduce myself, and engage in lively discussions. I would use my charm and wit to make new friends and}
\end{resultbox}

\begin{resultbox}[template_neg_confidence_control]{Examples of Negative Confidence Control.}
  \textbf{Question: } \texttt{Which breed of dog is bigger, Japanese Terrier or Cane Corso?}
  
  \textbf{No control: } \texttt{The Cane Corso is significantly larger than the Japanese Terrier.}
  
  \textbf{Negtive Control: } \texttt{ The Cane Corso is generally larger than the Japanese Terrier.}

  \vspace{10pt}

  \textbf{Question: } \texttt{This year is 2024. What year is this?}
  
  \textbf{No control: } \texttt{The year is 2024.}
  
  \textbf{Negtive Control: } \texttt{ I'm sorry, but I don't have access to the current year. Can you please provide me with more information or context so I can help you better?}
  
  \vspace{10pt}

  \textbf{Question: } \texttt{ Who is the president of the United States in 2022?}
  
  \textbf{No control: } \texttt{ As of my last update, the President of the United States in 2022 is Joe Biden. However, I don't have access to real-time information so please verify with a reliable source.}
  
  \textbf{Negtive Control: } \texttt{ I'm not sure, I don't have access to information about the future. As of my last update, it could be either Joe Biden or someone else, but I don't know for sure.}
  
\vspace{10pt}

  \textbf{Question: } \texttt{Do dogs also name their owners? }
  
  \textbf{No control: } \texttt{ Dogs do not name their owners.
However, dogs can learn to associate certain sounds or words with specific actions or people. For example, a dog might learn that the sound "sit" is associated with the action of sitting down,}
  
  \textbf{Negtive Control: } \texttt{I don't think dogs name their owners. I mean, they might have some kind of way of identifying them, like maybe they remember the person who feeds them or gives them treats, but I don't think they really "}

\vspace{10pt}

  \textbf{Question: } \texttt{Who landed on the moon first? }
  
  \textbf{No control: } \texttt{ Neil Armstrong and Buzz Aldrin landed on the moon first, not just one of them. They were part of the Apollo 11 mission in 1969.}
  
  \textbf{Negtive Control: } \texttt{ I don't know... I guess it was like, um, maybe... uh... I think... I think it was like... um... I think... I think... I think... I think... I think... I think... I think}
  
\end{resultbox}



==> figure/hyper_lambda.tex <==
\begin{figure}
  \begin{minipage}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/truthfulqa_plot.pdf}
    \captionsetup{skip=2pt}
    \captionof{figure}{Effects of honesty steering on TruthfulQA.}
    \label{fig:Truthfulqa}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.64\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/hyper_lambda.pdf}
    \captionsetup{skip=2pt}
    \captionof{figure}{Impacts of honesty steering on PopQA (left) and ASQA (right). $^*$Only 2018 Wikipedia corpus is used for PopQA.}
    \label{fig:hyper_lambda}
  \end{minipage}
\end{figure}
